Recasting Residual-based Local Descriptors as Convolutional Neural Networks: an Application to Image Forgery Detection

Local descriptors based on the image noise residual have proven extremely effective for a number of forensic applications, like forgery detection and localization. Nonetheless, motivated by promising results in computer vision, the focus of the research community is now shifting on deep learning. In this paper we show that a class of residual-based descriptors can be actually regarded as a simple constrained convolutional neural network (CNN). Then, by relaxing the constraints, and fine-tuning the net on a relatively small training set, we obtain a significant performance improvement with respect to the conventional detector.

==> figure/fridrich.tex <==
\usetikzlibrary{shadows}
\usetikzlibrary{decorations.pathreplacing}
\begin{tikzpicture}[scale=1]
\tikzset{rett/.style={draw,thick,align=center,drop shadow,fill=white,minimum width=1.5cm,minimum height=1cm,rounded corners=0mm}};
\tikzset{rettSmall/.style={draw,thick,align=center,drop shadow,fill=white,minimum width=1.5cm,minimum height=.5cm,rounded corners=0mm}};
\tikzset{rettBig/.style={draw,thick,align=center,drop shadow,fill=white,minimum width=1.5cm,minimum height=4cm,rounded corners=0mm}};

% Griglie
 
\node (input) at (0,8.5) {\large $x_{i,j}$};
\node [rett](FF0) at (2,8.5) {\large  Residue};
\node [rett](SQ0) at (5.5,8.5) {\large Quantization\\  and Truncation};
\node [inner sep = 0cm, fill=black](SQ1) at (7.8,8.5) {};

\node [rettSmall](FF1) at (9.5,10) {\large $\delta_{i,j-2}$};
\node [rettSmall](FF2) at (9.5,9) {\large $\delta_{i,j-1}$};
\node [rettSmall](FF3) at (9.5,8) {\large $\delta_{i,j}$};
\node [rettSmall](FF4) at (9.5,7) {\large $\delta_{i,j+1}$};

\node [rettBig](CoderB) at (12,8.5) {};
\node [rotate=90](Coder) at (12,8.5) {\Large sub2ind};

\node [rettBig](HistB) at (15,8.5) {};
\node [thick,align=center,rotate=90](Hist) at (15,8.5) {\large compute\\ \Large Histogram};

\node [](h1) at (17.5,9.5) {\large $h_1$};
\node [](h2) at (17.5,9.0) {\large $h_2$};
\node [](h3) at (17.5,8.5) {\large $h_3$};
\node [](hC) at (17,8.0) {$\vdots$};
\node [](hN) at (17.5,7.5) {\large $h_K$};

\draw[very thick,->,out=0,in=180] (input)  edge (FF0) ;
\draw[very thick,->,out=0,in=180] (FF0)  edge node[above]{\large $r_{i,j}$}  (SQ0) ;
\draw[very thick,-  ,out=0,in=180] (SQ0) edge node[above]{\large $\widehat{r}_{ij}$}  (SQ1) ;
\draw[very thick,->,out=0,in=180] (SQ1) |- (FF1) ;
\draw[very thick,->,out=0,in=180] (SQ1) |- (FF2);
\draw[very thick,->,out=0,in=180] (SQ1) |- (FF3);
\draw[very thick,->,out=0,in=180] (SQ1) |- (FF4);
\draw[very thick,->,out=0,in=180] (FF1) edge ($ (CoderB)+(-0.75,1.5) $);
\draw[very thick,->,out=0,in=180] (FF2) edge ($ (CoderB)+(-0.75,0.5) $);
\draw[very thick,->,out=0,in=180] (FF3) edge ($ (CoderB)+(-0.75,-0.5) $);
\draw[very thick,->,out=0,in=180] (FF4) edge ($ (CoderB)+(-0.75,-1.5) $);
\draw[very thick,->,out=0,in=180] (CoderB)  edge node[above]{\large $q_{i,j}$}  (HistB) ;
\draw[very thick,->,out=0,in=180] ($ (HistB)+(0.75,1)  $) -- (h1);
\draw[very thick,->,out=0,in=180] ($ (HistB)+(0.75,0.5) $) -- (h2);
\draw[very thick,->,out=0,in=180] ($ (HistB)+(0.75,0)  $) -- (h3);
\draw[very thick,->,out=0,in=180] ($ (HistB)+(0.75,-1) $) -- (hN);

%------------------------
\draw (7.5,6) [dashed]rectangle (16.5,11);
\node (P1) at (12,5.5) {\Large histogram of co-occurrencese};


\end{tikzpicture}
